Tree-Based versus Hybrid Graphical-Textual Model Editors: An Empirical Study of Testing Specifications

Tree-based model editors and hybrid graphical-textual model editors have advantages and limitations when editing domain models. Data is displayed hierarchically in tree-based model editors, whereas hybrid graphical-textual model editors capture high-level domain concepts graphically and low-level domain details textually. We conducted an empirical user study with 22 participants to evaluate the implicit assumption of system modellers that hybrid notations are superior, and to investigate the tradeoffs between the default EMF-based tree model editor and a Sirius/Xtext-based hybrid model editor. The results of the user study indicate that users largely prefer the hybrid editor and are more confident with hybrid notations for understanding the meaning of conditions. Furthermore, we found that the tree editor provided superior performance for analysing ordered lists of model elements, whereas activities requiring the comprehension or modelling of complex conditions were carried out faster through the hybrid editor.

==> casestudies.tex <==
\subsection{KUKA Case Study}
The KUKA use case is an industrial case study used by KUKA AG in
gearbox manufacture \cite{kuka-deliverable}. This use case
incorporates mobile robots to assemble the gear boxes, together with
human workers surrounding the assembly cell who assist the process. In
testing we aim to guarantee the safety requirement that robots must
not generate hazards to the human operators during operation. The
primary safety consideration is to ensure that robots do not enter
regions which could cause a collision hazard to human operators placed
around the outside of the assembly cell frame. Under normal
circumstances, motion trajectories are pre-planned to ensure
conformity to this safety requirement. However, faults in
communication, sensing or motor/interlock actuation may lead to robots
malfunctioning and rotating in order to enter these forbidden areas.
The simulation scenario was supplied for testing by end users,
implemented using the TTS simulation platform \cite{tts-simulator}.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/ttsScreenshot.png}
    \caption{KUKA assembly case primary view in TTS simulator}
    % TODO: new diagram here of the complete simulation
    \label{fig:kuka-case-study}
\end{figure}

The requirements for the case study are illustrated in Table
\ref{table:caseStudyTTSReqs}. The layout of the assembly cell is
illustrated in Figure \ref{fig:kuka-case-study}. The primary safety
requirement R1 is that the safety zones which the robots are forbidden
to enter are as illustrated as blue cuboid regions (Z1, Z2, Z3) on the
right-hand side of the external cell frame in Figure
\ref{fig:kuka-case-study}. If the region surrounding the gripper of
the right-hand robot (green cylinder labelled ZR3200) collides with
these regions, it will trigger violations which will be tracked and
counted as towards the static safety violation metric. The output
metric $staticCollision$ is used to quantify R1 by tracking the number
of intervals in which a collisions of the gripper safety zone with any
safety zone occured. The interval length is set to 0.2 seconds, which
provides independence of the event rate of the simulation.

Following a safety analysis, we have identified the communication from
the controller to the robot arm joints as vulnerable to message
disruptions. Therefore, requirement R1 will be tested by applying
fuzzing, altering the target motion value for robot arm joints with
jitter around the intended point. A part of the fuzzing model
instantiated for the KUKA industrial use case is presented in Figure
\ref{FIG-DSL-TTS-EXAMPLE}. The operations
$attackJointR3200ProductMove\_Link1$ and
$attackJointR3200ProductMove\_Link0$ of the model illustrate this
fuzzing offset value change, using the \emph{RandomValueFromSet}
fuzzing operation to apply relative changes to the joint value time
series.
\begin{figure}[t]
	\centering
        \includegraphics[width=\linewidth]{figures/tts-model-example-partial}
	\caption{A fragment of the DSL example for the TTS use case
          showing selected metrics and fuzzing operations}
	\label{FIG-DSL-TTS-EXAMPLE}
\end{figure}


==> dsl.tex <==
\subsection{Fuzzing Domain-Specific Language}
This section defines the domain-specific language (DSL) metamodel used
in this study, that specifies the fuzzing space, fuzzing operations,
and associated results. Employing DSLs tailored to a specific domain
is a highly desirable technique for extending the applicability of
modern software and systems engineering, enabling non-expert users to
easily test systems using our framework
~\cite{casalaro2021model,bruyninckx2013brics,gerasimou2019towards}.
In this paper, we explore two syntaxes for this metamodel, a graphical
syntax using the Exceed tree-based editor, and a hybrid syntax
developed using Sirius.

\begin{figure*}[!tb]
\centering
\includegraphics[width=0.93\linewidth]{figures/dsl-metamodel.jpg}
  \caption{UML classes for the core elements of the testing space DSL}
  \label{FIG-TESTSPACE-DSL}
\end{figure*}

A UML diagram showing a fragment of the DSL with three of the main
classes included is presented in Figure \ref{FIG-TESTSPACE-DSL}. The
figure presents the TestingSpace, TestCampaign and Test
classes. TestingSpace is the DSL's root element, consists of a set of
permissible fuzzing operations (possibleOperations) that collectively
specify the boundaries of the potential fuzzing space that can be
explored. The testing space also includes performance metrics which
are used to quantify the robotic system performance in regards to
safety violations, which allow multi-objective optimisation of system
performance to be performed. 

The TestCampaign class specifies an experiment that can be performed
and sets parameters for a specific fuzzing experiment. A TestCampaign
references a choice of particular metrics to use in evaluating that
campaign. The includedOperations reference list permits selecting a
subset of fuzzing operations in order to constrain an experiment.  The
TestGenerationApproach allows the user to specify the parameters for
an experiment by selecting one of these subclasses. For example,
NSGAEvolutionaryAlgorithm allows an evolutionary experiment with the
NSGA-II algorithm \cite{nsga2}. The performedTests attribute is
populated during the execution of experiments, with Tests generated
and executed for that campaign. The resultSets attribute is also
populated as the experiments proceed.

The Test class represents one test configuration that can be applied
to the MRS, corresponding to a particular selection of fuzzing
operations. During execution of the Test, metric instances will also
be recorded and stored. The latter are represented by the containment
of MetricInstances, which record performance metric results for the
evaluation of that particular Test. This provides a record of the
impact of the fuzzing performed.

The FuzzingOperation class represents one specific fuzzing operation -
an entity which represents a specific strategy for making runtime
modifications or disruptions to the MRS. Subclasses of
FuzzingOperation represent specific semantics of this fuzzing
operation; for example, the PacketLossNetworkOperation class
represents probabilistic loss of a proportion of packets. Currently,
\emph{variableToAffect} is the main attribute used when setting up
variable subscriptions and defining the variables to which fuzzing
operations are applied. Other FuzzingOperation subclasses such as
RandomValueFromSetOperation permits the replacement of structured
parameters within a message with newly generated random values.

The CampaignResultSet class represents either the final outcome of a
particular campaign, or partial intermediate results obtained during
its execution. An enumeration, ResultSetStatus, which is set to either
FINAL or INTERMEDIATE, determines this status of a result set. Result
sets contain references to particular Tests that comprise the
results. For example, in an evolutionary experiment, the set of Tests
for a final result set would contain the Pareto front obtained during
an experiment. Intermediate result sets would allow the user to
monitor the progression of the experiments and examine the changes in
the front at particular generations as the experiment progresses.

\subsection{Condition-Based Fuzzing}
Condition-based fuzzing provides the ability to activate and
deactivate fuzzing based upon custom scenario-specific events,
potentially incorporating complex mission logic, spatial and geometric
properties. A condition is a logical expression built hierarchically
from comparison and logical operations, incorporating state variables
from the robotic system during mission execution. The values of
condition variables change dynamically during the execution of the
mission, with every variable value supplied from an equally named
performance metric. Conditions can restrict the search space, making
the evolution of testing campaigns more tractable.

Activation of a condition-based fuzzing record is controlled by start
and end conditions. For each fuzzing record in the inactive state, the
start conditions will be evaluated at runtime on every simulation
event in order to determine a boolean status. If the condition
evaluates to true, that fuzzing record will be set to active. Then,
for every applicable event, the fuzzing operation will be invoked to
transform the incoming events for that fuzzing record. Once activated,
the fuzzing record remains active until the end condition evaluates to
true. Once the end condition is satisfied, fuzzing is deactivated for
this record. We assume that conditions can only be activated once,
such that a record which is activated is no longer available to be
reactivated later.

A primary intent of our paper is to assess the comprehensibility of
various syntaxes for understanding the meaning of particular
expressions. The DSL fragment for condition expressions is contained
in a seperate package, and its presented in Figure
\ref{FIG-CONDITIONS-DSL}. The Condition class consists of an abstract
ConditionElement, which is either a BasicCondition or
CompositeCondition. A BasicCondition represents comparisons of a
ConditionVariable with a ConditionExpression, which is either a
ConditionVariable or ConditionInteger. The BinaryCompisonOperation is
either LESS\_THAN, GREATER\_THAN, or EQUALS. ConditionVariables
contain a reference to an associated Metric that supplies its value,
and ConditionIntegers merely the primitive integer. A
CompositeCondition contains two other ConditionElements in the left
and right branches, together with a BinaryLogicalOperation. These
logical operations permit either AND or OR operations, and allow the
nesting of condition expressions to be arbitrarily deep.

\begin{figure}[!tb]
\centering
\includegraphics[width=\linewidth]{figures/dsl-metamodel-conditions.jpg}
  \caption{UML classes for the core elements of the testing space DSL}
  \label{FIG-CONDITIONS-DSL}
\end{figure}

Since condition expressions are dynamically generated during fuzzing
experiments, they may produce complex multi-level expressions. In this
paper, a major aspect is to investigate how different DSL syntaxes
permit the comprehension of deeply nested condition expressions,
allowing the user to interpret their meanings. We will also
investigate how the syntaxes allow the users to manually modify these
syntaxes.

==> userthemes.tex <==
\subsubsection{Graphical/Tree Based Syntax}
\begin{itemize}
\item Good for quick exploration - especially faster with keyboard
\item Better for non-condition/simple expressions
\item Some users found it hard to understand modifying/defining complex conditions
\item Some users liked defining/modifying conditions
\item Makes ordering/containment of elements clearer

% From the user survey text
\item Concise and hierarchical order; lets you see entire system on single page
\item Would likely have better scalability as models enlarge
\item Some users commented on it giving more of a sense of control over the model
\item May be more useful than hybrid for non-experts in domain to understand metamodel
\item Potential improvements: graphical/meaningful icons, visual difference to different elements
\item Potential improvements: Clarify type of element, visually or by color coding
\item Potential improvements: more information visible at level of each element (without clicking on it)
\item Potential improvements: introduce textual representation into tree e.g. for conditions
\end{itemize}

\subsubsection{Hybrid Syntax}
\begin{itemize}

\item Generally text better for entering condition expressions, especially deep expressions      
\item Diagram view switching/multiple boxes layout could be annoying
\item Some users not clear on why they had to double-click+confirm to enter new view             
\item May not be scalable to larger results - automatic layout may help
% From the user survey text
\item Visual aspect of hybrid syntax (e.g. tool pallette, colours etc) helpful
\item Easier to find interdependencies / relationships between objects in DSL
\item Textual provides a representation similar to that of programming languages
\item Allows prioritisation of elements by re-ordering e.g. manually adjusting layout
\item Potential improvements; auto layout algorithms, e.g. arrange of place items clearly in specific zones
\item Potential improvements; remove brackets, or use single consistent bracket throughout
\item Potential improvements: Improved validation or tooltips for conditions
\item Potential improvements; add home button to return to root
\end{itemize}
                                                                                                                        
 

